SwapMoE: Serving Off-the-shelf MoE-based Large Language Models with Tunable Memory Budget

Mixture of experts (MoE) is a popular technique to improve capacity of Large Language Models (LLMs) with conditionally-activated parallel experts. However, serving MoE models on memory-constrained devices is challenging due to the large parameter size. Typical solutions such as memory swapping or expert pruning may lead to significantly higher latency or severe accuracy loss. In this paper, we introduce SwapMoE, a framework for efficient serving of MoE-based large language models with tunable memory budgets. The main idea of SwapMoE is to keep a small dynamic set of important experts, namely Virtual Experts, in the main memory for inference, while seamlessly maintaining how the Virtual Experts map to the actual experts. Experiments have shown that SwapMoE can reduce the memory footprint while maintaining reasonable accuracy. For example, on text summarization tasks with Switch Transformer, SwapMoE can reduce the memory consumption from 14.2 GiB to 4.7 GiB, together with 50\% latency reduction and a slight Rouge-2 score drop of 0.041.

==> tex/implementation.tex <==
\section{Implementation} \label{sec:implementation}

We implemented \name atop two popular MoE frameworks, Tutel~\cite{tutel:arxiv22:Changho} for Swin-MoE, and Huggingface Transformers~\cite{wolf2019huggingface} for Switch Transformer~\cite{switch_moe:jmlr22:Fedus} and GPTSAN~\cite{gptsan}, with 4k LoC added. 
% \yuanchun{refs}
% \yuanchun{check:}
Tutel uses customized operators for MoE layers, which employ token padding techniques to enhance load balancing and shape alignment between experts. Since the main focus of this paper is not to address the impact of padding, we directly adopted the token padding techniques used in Tutel.
% Specifically, in a specific MoE layer, the number of tokens processed by different experts is padded to be the same, which reduces communication overhead by avoiding alignment issues between tokens. However, the drawback is that if an expert processes a small number of tokens, it may introduce additional computation on padding tokens. Since the main focus of this paper is not to address the impact of padding, we directly adopted the token padding techniques used in Tutel.

\textbf{Efficient implementation of \core.} 
% \kongrui{How we use torch.copy\_ to reduce more memory footprint}
% 为了减少experts换入换出main memory所带来的额外memory footprint，我们将\core抽象为指针的概念。如Figure~\ref{figure:expert_buffer_update}所示，\core是一直存放在main memory，这部分内存是一开始就分配好并且不需要重新分配的，\core所包含的experts weights就是它所指向的important experts。当我们需要对\core中的experts进行更新时，我们采用Pytorch中的torch.copy\_ API来进行expert weights传输，无需占用额外的main memory，相当于更新了\core所指向的experts.
To minimize the additional memory footprint caused by experts' swapping in and out of main memory, we abstract \core as a pointer concept. \core remains stored in main memory, a portion of memory that is pre-allocated and does not require reallocation. The expert weights contained in \core are those to which it points. When loading experts to \core are necessary, we utilize the \textit{torch.copy\_} API in PyTorch for transferring expert weights, thereby avoiding the need for additional main memory allocation. This process effectively updates the experts to which \core points.

\textbf{Genetic algorithm configurations.} We provide the parameters used in the genetic algorithm to search the optimal \core configuration. The population size is 50, the mutation rate is 0.5, the crossover rate is 0.01, and the number of generations is 5000.
% \yuanchun{The hyperparameters should be in the implementation (or later in this subsection). Here you need to primarily describe the design (constraints, cross-over, mutation, etc.).}
To ensure feasible results, we set the lower bound of the search space to 1 and the upper bound to the total number of experts in the MoE layer. 

\textbf{Profiling data processing.}
During the implementation of \name, we utilized 10\% of the test data as profiling data. To have a sufficiently long profiling data set, we replicated this 10\% of data multiple times and concatenated the beginning with the end. It is worth mentioning that label is not required for all the data in the online phase.
